PAT: Parameter-Free Audio-Text Aligner to Boost Zero-Shot Audio Classification

Audio-Language Models (ALMs) have demonstrated remarkable performance in zero-shot audio classification. In this paper, we introduce PAT (Parameter-free Audio-Text aligner), a simple and training-free method aimed at boosting the zero-shot audio classification performance of CLAP-like ALMs. To achieve this, we propose to improve the cross-modal interaction between audio and language modalities by enhancing the representations for both modalities using mutual feedback. Precisely, to enhance textual representations, we propose a prompt ensemble algorithm that automatically selects and combines the most relevant prompts from a datastore with a large pool of handcrafted prompts and weighs them according to their relevance to the audio. On the other hand, to enhance audio representations, we reweigh the frame-level audio features based on the enhanced textual information. Our proposed method does not require any additional modules or parameters and can be used with any existing CLAP-like ALM to improve zero-shot audio classification performance. We experiment across 18 diverse benchmark datasets and 6 ALMs and show that the PAT outperforms vanilla zero-shot evaluation with significant margins of 0.42%-27.0%. Additionally, we demonstrate that PAT maintains robust performance even when input audio is degraded by varying levels of noise. Our code will be open-sourced upon acceptance.

==> main_music_results.tex <==
\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{@{}ccccccccccc@{}}
\toprule
\textbf{Model}                    & \textbf{Evaluation} & \textbf{GTZAN} & \textbf{Medley} & \textbf{NSynth Inst} & \textbf{NSynth Src} & \textbf{MSDB} & \textbf{Beijing Op.} & \textbf{Mri. St} & \textbf{Mri. To} & \textbf{Avg} \\ \midrule
\multirow{4}{*}{LAION CLAP}       & ZS                  & 43.4           & 82.5            & 37.2                 & 37                  & 55.6          & 45.34                & 10.81            & 25.1             & x            \\
                                  & PAT                 & 54.2           & 92              & 38                   & 41                  & 66            & 68.64                & 37.35            & 34.38            & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
\multirow{4}{*}{LAION CLAP Music} & ZS                  & 63.92          & 87.88           & 31.67                & 43.92               & 73.2          & 75                   & 47.4             & 27.59            & x            \\
                                  & PAT                 & 55.93          & 94.3            & 36.49                & 46.38               & 69.2          & 75.42                & 35.08            & 31.62            & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
\multirow{4}{*}{MS CLAP 2022}     & ZS                  & GTZAN          & Medley          & 26.26                & 37.06               & MSDB          & 54.24                & 14.5             & 16.5             & x            \\
                                  & PAT                 & GTZAN          & Medley          & 29.63                & 41.45               & MSDB          & 73.72                & 14.8             & 15.63            & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
\multirow{4}{*}{MS CLAP 2023}     & ZS                  & 56.24          & 95              & 63.3                 & 49.7                & 61.2          & 71.19                & 44.09            & 22.02            & x            \\
                                  & PAT                 & 58.56          & 96.28           & 66.3                 & 61.45               & 62.4          & 71.61                & 47.12            & 26.18            & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
\multirow{4}{*}{Wav2Clip}         & ZS                  & GTZAN          & 51.95           & 24.39                & 36.72               & 51.6          & 26.69                & 8.46             & 15.57            & x            \\
                                  & PAT                 & GTZAN          & 59.01           & 21.72                & 42.01               & 49.2          & 34.32                & 5.76             & 19.27            & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
\multirow{4}{*}{AudioClip}        & ZS                  & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & PAT                 & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o WPE             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\
                                  & w/o CMA             & GTZAN          & Medley          & NSynth Inst          & NSynth Src          & MSDB          & Beijing Op.          & Mri. St          & Mri. To          & x            \\ \bottomrule
\end{tabular}}
\caption{Main results}
\label{tab:main_result}
\end{table*}

==> main_sound_results.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.8\textwidth}{!}{\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Model}                    & \textbf{Evaluation} & \textbf{ESC-50} & \textbf{USD-8K} & \textbf{TUT} & \textbf{VS} & \textbf{DCASE} & \textbf{Gunshot Tri} & \textbf{Avg} \\ \midrule
\multirow{4}{*}{LAION CLAP}       & ZS                  & 89              & 76              & 36           & 78.2        & 44.88          & 10.23                & x            \\
                                  & PAT                 & 93              & 80              & 39           & 80          & 50.81          & 22.72                & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
\multirow{4}{*}{LAION CLAP Music} & ZS                  & 85.6            & 28.09           & 28.09        & 74.46       & 56.76          & 13.64                & x            \\
                                  & PAT                 & 92.65           & 39.93           & 39.93        & 78.91       & 55.94          & 29.52                & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
\multirow{4}{*}{MS CLAP 2022}     & ZS                  & ESC-50          & USD-8K          & 24.44        & VS          & 13.93          & 17.05                & x            \\
                                  & PAT                 & ESC-50          & USD-8K          & TUT          & VS          & 23.77          & 23.86                & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
\multirow{4}{*}{MS CLAP 2023}     & ZS                  & 91.8            & 77.7            & 45           & 79          & 45.9           & 25                   & x            \\
                                  & PAT                 & 94.8            & 82.5            & 47           & 79.6        & 39.96          & 25                   & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
\multirow{4}{*}{Wav2Clip}         & ZS                  & ESC-50          & 24.35           & 11.54        & 17.54       & 9.63           & 20.19                & x            \\
                                  & PAT                 & ESC-50          & 33.47           & 15.18        & 17.23       & 17.21          & 25.7                 & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
\multirow{4}{*}{AudioClip}        & ZS                  & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & PAT                 & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o WPE             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\
                                  & w/o CMA             & ESC-50          & USD-8K          & TUT          & VS          & DCASE          & Gunshot Tri          & x            \\ \bottomrule
\end{tabular}}
\caption{Main results}
\label{tab:main_result}
\end{table*}
